Dorylus: Affordable, Scalable, and Accurate GNN Training with Distributed CPU Servers and Serverless Threads

A graph neural network (GNN) enables deep learning on structured graph data. There are two major GNN training obstacles: 1) it relies on high-end servers with many GPUs which are expensive to purchase and maintain, and 2) limited memory on GPUs cannot scale to today's billion-edge graphs. This paper presents Dorylus: a distributed system for training GNNs. Uniquely, Dorylus can take advantage of serverless computing to increase scalability at a low cost. The key insight guiding our design is computation separation. Computation separation makes it possible to construct a deep, bounded-asynchronous pipeline where graph and tensor parallel tasks can fully overlap, effectively hiding the network latency incurred by Lambdas. With the help of thousands of Lambda threads, Dorylus scales GNN training to billion-edge graphs. Currently, for large graphs, CPU servers offer the best performance-per-dollar over GPU servers. Just using Lambdas on top of CPU servers offers up to 2.75x more performance-per-dollar than training only with CPU servers. Concretely, Dorylus is 1.22x faster and 4.83x cheaper than GPU servers for massive sparse graphs. Dorylus is up to 3.8x faster and 10.7x cheaper compared to existing sampling-based systems.

==> eval-old-performance-and-costs.tex <==
\mysubsection{Performance and Costs\label{sec:scalability}}
This subsection focuses on understanding the scalability, efficiency, and cost of \tool. Comparisons with existing systems on smaller graphs are discussed in \S\ref{sec:comparison}. For a thorough comparison, we developed two other variants, one (GPU) that uses GPUs on each GS to perform tensor and graph computation and a second (CPU) that does so with only CPUs. Note that these two variants were built on top of the \tool architecture, which enables scalability by separating the tensor- and graph-parallel computation.

\begin{table*}[t]
    \setlength\arrayrulewidth{.5pt}
    \scriptsize\centering
   \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{c|c||c|c|c|c|c||c|c|c|c|c}
        \toprule
			& \textbf{CPU} & \multicolumn{5}{c||}{\textbf{Performance (seconds)}} & \multicolumn{5}{c}{\textbf{Cost (\$)}}  \\ \cmidrule{3-7} \cmidrule{8-12}
        \textbf{Graph} & \textbf{Environment} &
        \textbf{Pipe} & \textbf{Async($s$=0)}   & \textbf{Async($s$=1)} & \textbf{CPU} &  \textbf{GPU} &  \textbf{Pipe} & \textbf{Async($s$=0)}   & \textbf{Async($s$=1)} & \textbf{CPU} &  \textbf{GPU}\\ \midrule
         \multirow{2}{*}{Reddit-small}    &  c5.2xlarge (2)  &  914.3 & \textbf{860.6} & 890.1 & 1005.4 & \textbf{162.9} & 0.21 & \textbf{0.20} & 0.21 & \textbf{0.19} & 0.28 \\
                    &  c5n.2xlarge (2)   & 915.0 & \textbf{887.1} & 933.0 & 1018.4 & \textbf{162.9} & 0.25 & \textbf{0.25} & 0.26 & \textbf{0.24} & 0.28 \\ \midrule
        \multirow{2}{*}{Amazon}  & c5.2xlarge (8)  & 589.4 & \textbf{559.7} & 651.7 & 703.4 & \textbf{385.3} & \textbf{0.82} & 0.89 & 1.18 & \textbf{0.53} & 2.62 \\ 
                    &  c5n.2xlarge (8)  & 534.5 & \textbf{512.7} & 684.4 & 710.2 & \textbf{385.3} & 0.84 & \textbf{0.79} & 1.16 & \textbf{0.68} & 2.62  \\ \midrule
       
        \multirow{2}{*}{Reddit-large}     &  c5.4xlarge (12)     &  \textbf{1034.8} & 1076.0  & 1437.7  & 1320.8   & \textbf{324.9}   &  \textbf{1.44} & \textbf{1.48} & 1.92 & 1.50& 3.31 \\
                    &  c5n.4xlarge (12)    &  \textbf{1020.1} & 1061.2  & 1408.8 & 1290.5 & \textbf{324.9}   &  \textbf{1.69} & \textbf{1.76} & 2.32 & 1.85& 3.31\\ \midrule            
       Friendster    &  c5n.4xlarge (32)    & 1773.4 & \textbf{1213.9} & 1811.0 & 1990.8 & \textbf{1490.4} & 18.2 & \textbf{16.4} & 19.9 & \textbf{15.3} & 40.5
                    %&  cn5.2xlarge (8)    &       &     &   &    &       &     &  & & & 
        \\\bottomrule    \end{tabular}
   \end{adjustbox}
    \vspace{-1.5em}
    \caption{Overall GCN performance and costs between five systems: the sync version of \tool (pipe), two async versions with different staleness values (async, s=0 and s=1), the CPU-based (CPU), and the GPU-based backend (GPU). Reported are their environments (\ie, EC2 instance types and numbers of instances used), running times to reach the same accuracy, as well as the costs on EC2. The lowest and second-lowest times/costs are highlighted for each graph. \label{tab:gcn-overall}}
    \vspace{-1.5em}
\end{table*}

\begin{table*}[t]
    \setlength\arrayrulewidth{.5pt}
    \scriptsize\centering
   \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{c|c||c|c|c|c|c||c|c|c|c|c}
        \toprule
			& \textbf{CPU}& \multicolumn{5}{c||}{\textbf{Performance (seconds)}} & \multicolumn{5}{c}{\textbf{Cost (\$)}}  \\ \cmidrule{3-7} \cmidrule{8-12}
        \textbf{Graph} & \textbf{Environment} &
        \textbf{Pipe} & \textbf{Async($s$=0)}   & \textbf{Async($s$=1)} & \textbf{CPU} &  \textbf{GPU} &  \textbf{Pipe} & \textbf{Async($s$=0)}   & \textbf{Async($s$=1)} & \textbf{CPU} &  \textbf{GPU}\\ \midrule
         \multirow{2}{*}{Reddit-small}    
         &  c5.2xlarge (10)     & 630.3 & \textbf{496.3} & 570.2 & 1270.4 & \textbf{130.9} & \textbf{0.96} & 1.15 & 1.31 & 1.20 & \textbf{1.11}\\
                    &  c5n.2xlarge (10)  & 644.9 & \textbf{564.7} & 569.1 & 1364.4 & \textbf{130.9} & \textbf{1.25} & 1.35 & 1.44 & 1.64 & \textbf{1.11}\\ \midrule
        \multirow{2}{*}{Amazon}  
        & c5.2xlarge (12)    & 1436.0 & \textbf{930.2} & \textbf{1014.6} & 2232.3 & 1039.2 & 3.84 & \textbf{2.88} & 3.06 & \textbf{2.53} & 10.6 \\ 
                    &  c5n.2xlarge (12)   & 1368.8 & \textbf{853.4} & \textbf{903.3} & 2092.7 & 1039.2 & 3.97 & \textbf{2.67} & 3.15 & \textbf{3.01} & 10.6 % \\\midrule
       % \multirow{2}{*}{Reddit-large}     &  cn5.2xlarge (8)    &       &     &   &    &       &     &  & & & \\
       %             &  c5n.2xlarge (8)    &       &     &   &    &       &     &  & & & \\ \midrule            
       % Friendster    % &  cn5.2xlarge (8)    &       &     &   &    &       &     &  & & & \\
      %              &  c5n.2xlarge (8)    &       &     &   &    &       &     &  & & & 
        \\\bottomrule    \end{tabular}
   \end{adjustbox}
    \vspace{-1.5em}
    \caption{Overall GAT performance and costs between the five systems over \codeIn{Reddit-small} and \codeIn{Amazon}. \label{tab:gat-overall}}
    \vspace{-2.2em}
\end{table*}

% old data
\begin{comment}
\begin{table*}[t]
    \setlength\arrayrulewidth{.5pt}
    \scriptsize\centering
   \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{c|c||c|c|c|c|c||c|c|c|c|c}
        \toprule
			& \textbf{CPU} & \multicolumn{5}{c||}{\textbf{Performance (seconds)}} & \multicolumn{5}{c}{\textbf{Cost (\$)}}  \\ \cmidrule{3-7} \cmidrule{8-12}
        \textbf{Graph} & \textbf{Environment} &
        \textbf{Pipe} & \textbf{Async($s$=0)}   & \textbf{Async($s$=1)} & \textbf{CPU} &  \textbf{GPU} &  \textbf{Pipe} & \textbf{Async($s$=0)}   & \textbf{Async($s$=1)} & \textbf{CPU} &  \textbf{GPU}\\ \midrule
         \multirow{2}{*}{Reddit-small}    &  c5.2xlarge (2)    &   1469.1 & \textbf{1449.3}  & 1971.2 & 1549.6  & \textbf{147.7}  &  \textbf{0.17}  & \textbf{0.16} & 0.23 & 0.29 & 0.25 \\
                    &  c5n.2xlarge (2)   & 1356.8   & \textbf{1325.4} & 1816.9  &  1416.0& \textbf{147.7} & 0.19  & \textbf{0.18}  & 0.26 & \textbf{0.17} & 0.25\\ \midrule
        \multirow{2}{*}{Amazon}  & c5.2xlarge (8)  &  857.8  &  \textbf{844.1}  &  1139.5 &  1058.6  &  \textbf{755.4} &  \textbf{1.21}  & 1.33 & 1.82 & \textbf{0.80} & 5.13 \\ 
                    &  c5n.2xlarge (8)  &  771.9 & \textbf{735.5}  & 935.6  & 1002.1   & \textbf{755.4}   & \textbf{1.23} & 1.28  &  1.59 & \textbf{0.96} & 5.14  \\ \midrule
       
        \multirow{2}{*}{Reddit-large}     &  c5.4xlarge (12)     &  \textbf{1034.8} & 1076.0  & 1437.7  & 1320.8   & \textbf{324.9}   &  \textbf{1.44} & \textbf{1.48} & 1.92 & 1.50& 3.31 \\
                    &  c5n.4xlarge (12)    &  \textbf{1020.1} & 1061.2  & 1408.8 & 1290.5 & \textbf{324.9}   &  \textbf{1.69} & \textbf{1.76} & 2.32 & 1.85& 3.31\\ \midrule            
       Friendster    &  c5n.4xlarge (32)    &  \textbf{1773.4}   &  \textbf{1280.7} & 1849.3  &  1990.8  & 2768.3   &  18.2  & \textbf{17.3} & 20.4 & \textbf{15.3} & 75.3
                    %&  cn5.2xlarge (8)    &       &     &   &    &       &     &  & & & 
        \\\bottomrule    \end{tabular}
   \end{adjustbox}
    \vspace{-1.5em}
    \caption{Overall GCN performance and costs between five configurations of \tool: the sync version of \tool (Pipe), two async versions with different staleness values (Async, s=0 and s=1), the CPU-based version (CPU), and the GPU-based version (GPU). Reported are their environments (\ie, EC2 instance types and numbers of instances used), running times to reach the same accuracy, as well as costs on EC2. The lowest and second-lowest times/costs are highlighted for each graph. \label{tab:gcn-overall}}
    \vspace{-1.5em}
\end{table*}

\begin{table*}[t]
    \setlength\arrayrulewidth{.5pt}
    \scriptsize\centering
   \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{c|c||c|c|c|c|c||c|c|c|c|c}
        \toprule
			& \textbf{CPU}& \multicolumn{5}{c||}{\textbf{Performance (seconds)}} & \multicolumn{5}{c}{\textbf{Cost (\$)}}  \\ \cmidrule{3-7} \cmidrule{8-12}
        \textbf{Graph} & \textbf{Environment} &
        \textbf{Pipe} & \textbf{Async($s$=0)}   & \textbf{Async($s$=1)} & \textbf{CPU} &  \textbf{GPU} &  \textbf{Pipe} & \textbf{Async($s$=0)}   & \textbf{Async($s$=1)} & \textbf{CPU} &  \textbf{GPU}\\ \midrule
         \multirow{2}{*}{Reddit-small}    
         &  c5.2xlarge (10)     &  620.3  & \textbf{496.3}  & 570.2 & 1267.2  & \textbf{130.9}  & \textbf{0.96}    & 1.15 & 1.30 & 1.20 & \textbf{1.11}\\
                    &  c5n.2xlarge (10)  & 644.8  & \textbf{564.7}   & 569.1  & 1364.4  & \textbf{130.9}  &  \textbf{1.25}   & 1.35 & 1.44  & 1.64 & \textbf{1.11}\\ \midrule
        \multirow{2}{*}{Amazon}  
        & c5.2xlarge (12)    &  1435.9     &   \textbf{930.2}  & \textbf{1014.6}   & 2232.3   & 1045.1      & 3.84    &  \textbf{2.88} & 3.06 &  \textbf{2.53} & 10.6 \\ 
                    &  c5n.2xlarge (12)   &  1368.8 &  \textbf{853.4}  & \textbf{903.3}   & 2090.6& 1045.1  & 3.97  &  \textbf{2.67} & 3.15 & \textbf{2.53} & 10.6 % \\\midrule
       % \multirow{2}{*}{Reddit-large}     &  cn5.2xlarge (8)    &       &     &   &    &       &     &  & & & \\
       %             &  c5n.2xlarge (8)    &       &     &   &    &       &     &  & & & \\ \midrule            
       % Friendster    % &  cn5.2xlarge (8)    &       &     &   &    &       &     &  & & & \\
      %              &  c5n.2xlarge (8)    &       &     &   &    &       &     &  & & & 
        \\\bottomrule    \end{tabular}
   \end{adjustbox}
    \vspace{-1.5em}
    \caption{Overall GAT performance and costs between the five systems over \codeIn{Reddit-small} and \codeIn{Amazon}. \label{tab:gat-overall}}
    \vspace{-2.2em}
\end{table*}
\end{comment}

\MyPara{Systems Considered.} We ran five variants of \tool: synchronous version with full intra-epoch pipelining (pipe), two asynchronous versions with the staleness value being 0 and 1 (async, $s$=0 and $s$=1), CPU, and GPU over these four graphs. Pipe synchronizes at each \codeIn{Gather} --- a vertex cannot go forward until all its neighbors have their latest values scattered. As a result, all vertex intervals have to be in the same epoch. However, inside each epoch, pipelining is enabled, and hence the processing of different tasks is fully overlapped. Async enables both pipelining and asynchrony (\ie, stashing weights and using stale values at GA). When the staleness value is $s$ = 0, \tool allows a vertex to use a stale value from a neighbor as long as the value is computed in the same epoch (\eg, can be in a previous layer). In other words, if the value is generated from a previous epoch, it is not allowed to be used and synchronization is needed. 

Note that async ($s$=0) is fundamentally different from pipe in that pipe does \emph{not} allow different intervals to be in different epochs (because GA always waits for the latest values from neighbors), whereas in async ($s$=0) an interval $i$ can be many epochs ahead of  another interval $j$ as long as the neighbor intervals of $i$ are as fast as $i$ (\ie, in the same epoch). Similarly, async ($s$=1) allows GA to use neighbor values if they are generated in either the current or the previous epoch. 

For each graph, we picked the number of servers such that they have just enough memory to hold the graph data and their tensors. 
For example, for \codeIn{Amazon}, eight c5.2xlarge servers (with 16GB memory) provide enough memory to hold the data, while for \codeIn{Friendster}, we need 32 c5n.4xlarge instances (with a total of 1344GB memory).
% For example, for \codeIn{Reddit-small}, two c5.2xlarge servers (with 16GB memory) provide enough memory to hold the data, while for \codeIn{Friendster}, we need 32 c5n.4xlarge instances (with a total of 1344GB memory). 
For each graph, the number of GPU servers used in p3 is the same as that of CPU servers. The goal here is to train a model with the minimum amount of resources. For \codeIn{Friendster}, we only ran it on c5n.4xlarge servers due to the long running time and high training costs.  Of course, using more servers will lead to better performance and higher costs. An evaluation with different numbers of servers will be discussed shortly in \S\ref{sec:cost-efficiency}. 

\begin{figure*}[t]
\centering
\scriptsize
\begin{tabular}{ccc}
\includegraphics[scale=.3]{figs/progress-reddit-small.pdf}
     &  
\includegraphics[scale=.3]{figs/progress-amazon.pdf}     
    &
\includegraphics[scale=.3]{figs/progress-reddit-large.pdf}\\
 (a) \codeIn{Reddit-small} &  (b) \codeIn{Amazon} & (c) \codeIn{Reddit-large}  \\
 \textbf{R[$s$=0]:1.00, R[$s$=1]:1.07, Accuracy:94.96\%} & \textbf{R[$s$=0]:1.09, R[$s$=1]:1.57, Accuracy:64.08\% } &  \textbf{R[$s$=0]:1.14, R[$s$=1]:1.58, Accuracy:60.07\%}
 \end{tabular}
 \vspace{-1.5em}
 \caption{Asynchronous progress for GCN: each line shows the change of the accuracy \emph{normalized} to the final accuracy achieved (\ie, \textbf{94.96\%}, \textbf{64.08\%}, \textbf{60.07\%} for the three graphs). \codeIn{Friendster} is not included because it does not come with meaningful features and labels. %Each dot indicates 5 epochs.
 \label{fig:async-progress}}
 \vspace{-1.8em}
 \end{figure*}
 
Due to the use of asynchrony, it may take the asynchronous version of \tool more epochs to reach the same accuracy as pipe, CPU, and GPU. To enable a fair comparison, we first ran \tool-pipe until convergence (\ie, the difference of the model accuracy between consecutive epochs is within 0.001, unless otherwise stated) and then used this accuracy as the target accuracy to run async when collecting training time. However, this approach does not work for \codeIn{Friendster}, because it uses randomly generated features/labels and hence accuracy is not a meaningful target. To solve this problem, we computed an average ratio, across the other three graphs, between the numbers of epochs needed for async and pipe, and used this ratio to estimate the training time for \codeIn{Friendster}. For example, this ratio is 1.08 for $s$=0 and 1.41 for $s$=1. As such, we let async ($s$=0) run N$\times$1.08 epochs and async ($s$=1) run N$\times$1.41 epochs when measuring performance for \codeIn{Friendster} where $N$ is the number of epochs pipe runs.  

\MyPara{Overall Performance and Costs.} The performance and costs for each system variant are reported in Table~\ref{tab:gcn-overall} for GCN and Table~\ref{tab:gat-overall} for GAT. GAT training was done only on two graphs (\codeIn{Reddit-small} and \codeIn{Amazon}) because GAT has very intensive AE computation, leading to many more servers required and much longer training time than GCN. We did not train GAT on the two billion-edge graphs, but this is \emph{not} because of any limitation in our system, but rather too long a training time we could not wait. Note that GAT is a recently developed model~\cite{gtn-nips19} and its state-of-the-art training system can only process graphs with thousands of edges.
%(\eg, Cora, Citeseer, or Pubmed). 



For each configuration, we highlight the two lowest training times and two lowest costs. As expected, the GPU version has the best performance, followed by async ($s$=0) in most cases. The performance of pipe is worse than async ($s$=0), but on par with that of async ($s$=1). CPU has the worst performance in most cases. In terms of training costs, CPU has the lowest costs in most cases, followed by pipe and async ($s$=0), whose costs are very close. The costs of GPU are the highest. 



%Our first observation is that the larger a graph is, the more performance benefit \tool provide. For example, for \codeIn{Reddit-small}, the smallest graph in our dataset, \tool-GPU is almost 10$\times$ faster than \tool because the graph and tensor data can easily fit into GPU's memory. When the graph size increases, more servers are needed and hence GPUs on each server need to wait during the \codeIn{Scatter} phase, leading to inefficiencies. In \tool, the \codeIn{Scatter} phase overlaps with other phases due to the computation separation. However, \tool-GPU performs all tasks in GPUs, and as such, it has to wait when servers communicate. This explains why \tool-async ($s$=0) outperforms \tool-GPU in a number of cases (\eg, \codeIn{Amazon}, \codeIn{Friendster}). 

\MyPara{Observations.} 
\underline{Our first observation} is that the more sparse the graph, the more useful \tool is. Sparsity of each graph can be seen from the average vertex degree reported in Table~\ref{tab:graphs}. As shown, \codeIn{Amazon} and \codeIn{Friendster} are much more sparse than \codeIn{Reddit-small} and \codeIn{Reddit-large}, and the graphs over which the performance of async ($s$=0) is better than or on par with that of GPU. There are two major reasons:

%For the largest graph \codeIn{Friendster}, GPU is slower than the other variants. We carefully investigated our results and found two important reasons.
First, for all versions, the fraction of time on \codeIn{Scatter} is significantly larger when training over \codeIn{Friendster} and \codeIn{Amazon} than \codeIn{Reddit-small} and \codeIn{Reddit-large}. This is, at first sight, counter-intuitive because one would naturally expect less efforts on inter-partition communications for sparse graphs than dense graphs. A thorough inspection discovered that the \codeIn{Scatter} time actually depends on a \emph{combination} of the number of ghost vertices and inter-partition edges. For the two Reddit graphs, they have many inter-partition edges, but very few ghost vertices, because (1) their $|V|$ is small and (2) many inter-partition edges come from/go to the same ghost vertices due to their high vertex degrees. 

Second, \codeIn{Scatter} (\eg, buffering, sending and receiving) takes much longer time in GPU clusters. Moving ghost data between GPU memories on different nodes is much slower than data transferring between CPU memories. 
%Furthermore, \codeIn{Scatter} is executed by CPUs on GSes even if a GPU backend is used.
%It turns out that p3 -- EC2's highest-end GPU server family -- is not optimized for CPUs. p3 uses Intel Xeon Skylake processors (2.3GHz) while c5 -- the compute-optimized family -- uses Xeon Cascade with maximum single core frequency of 3.9GHz.  
As a result, GPU's poor performance is due to a combinatorial effect of these two factors: \tool scatters significantly more data for \codeIn{Friendster} and \codeIn{Amazon}, which amplifies the negative impact of poor scatter performance in a GPU cluster. 
%We could not find an instance type with both optimized CPUs and GPUs.
% The second reason is that \codeIn{Scatter} (\eg, data buffering, sending and receiving) is executed by CPUs on GSes even if a GPU backend is used. It turns out that p3 -- EC2's highest-end GPU server family -- is not optimized for CPUs. p3 uses Intel Xeon Skylake processors (2.3GHz) while c5 -- the compute-optimized family -- uses Xeon Cascade with maximum single core frequency of 3.9GHz.  GPU's poor performance is due to a combinatorial effect of these two factors: \tool scatter significantly more data for \codeIn{Friendster} and \codeIn{Amazon}, which amplifies the negative impact of the poor CPU performance on p3 machines. We could not find an instance type with both optimized CPUs and GPUs.

\underline{Our second observation} is that too large a staleness value leads to slow convergence and poor performance, although the per-epoch time reduces (see the per-epoch times in Figure~\ref{fig:per-epoch}). This explains why async ($s$=0) outperforms async ($s$=1) by a large margin. Async ($s$=0) has a performance gain over pipe due to asynchrony.  
%The effectiveness of asynchronous \codeIn{Gather} depends largely on weight stashing. Significant delays in convergence (20\%-30\%) were observed when weight stashing was disabled.% (these results are not shown in the paper due to space constraints).  

\underline{Our third observation} is that improving the networking bandwidth always leads to better performance (10\%-15\%), but not necessarily lower costs, due to the higher price of networking-enhanced instances.  

\underline{Our last observation} is that Lambda threads are more effective in boosting performance for GAT than GCN. This is because GAT includes an additional AE task, which performs intensive per-edge tensor computation and thus benefits significantly from a high degree of parallelism. 

\underline{Overall}, async ($s$=0) is about \textbf{1.51$\times$} slower than GPU and \textbf{1.74$\times$} faster than CPU, \textbf{1.234$\times$} faster than pipe, \textbf{1.233$\times$} than async ($s$=1). In terms of cost, it is \textbf{2.33$\times$} cheaper than GPU, and \textbf{only 1.004$\times$} more expensive than CPU.%\footnote{Calculated as averages normalized by numbers of \tool-async(s=0).}
\begin{comment}
\underline{Overall}, Dorylus-async ($s$=0) is about \textbf{2.5$\times$} slower than GPU and \textbf{2.1$\times$} faster than CPU. In terms of cost, it is \textbf{3.3$\times$} cheaper than GPU, and \textbf{1.2$\times$} more expensive than CPU.
\end{comment}

\begin{figure}[!ht]
\vspace{-.5em}
\centering
\includegraphics[scale=.5]{figs/per-epoch-time.pdf}
\vspace{-1.2em}
\caption{\je{Change to line graph.} Per-epoch GCN time normalized to that of pipe. \label{fig:per-epoch}}
\vspace{-1.5em}
\end{figure}

\MyPara{Cost-Benefit.} Note that in this set of experiments, \tool uses more CPU resources via Lambdas than the CPU-based backend. A more fair comparison would be to run the CPU backend with additional servers that offer equivalent compute to Lambdas. However, the number of Lambdas is dynamically tuned in our setting. In addition, each Lambda has much weaker compute than a typical CPU instance in any EC2 family, making it impossible to find the right number of equivalent CPU instances.  We carefully address this issue with two actions. First, we define a new metric \emph{cost-benefit} as the multiplication of the training time and monetary cost. This metric considers the amount of resources (reflected by the cost) and the gains over them (reflected by the time), putting our comparisons in a more sensible context. Figure~\ref{fig:cost-benefit} shows our results. 
\hx{Comparison results!}

Second, we increased the number of CPU servers and cross-compared the performance of all settings. These results will be discussed in \S\ref{sec:scalability}.


\MyPara{Training Progress.} Figure~\ref{fig:async-progress} reports the GCN training progress for each version of \tool, that is, how many epochs it took for a version to reach the target accuracy. Annotated with each figure are two ratios: R[$s$=0] and R[$s$=1], representing the ratio between the number of epochs needed by async ($s$=0/1) and that by \tool-pipe to reach the same target accuracy. On average,  async ($s$=0/1) increases the number of epochs by 8\%/41\%. 

Figure~\ref{fig:per-epoch} compares the per-epoch running time of async ($s$=0/$s$=1), CPU, and GPU, normalized to that of pipe. As expected, async has lower per-epoch time; in fact, async ($s$=0) achieves almost the same reduction ($\thicksim$15\%) in per-epoch time as $s$=1. This indicates that choosing a large staleness value has little usefulness --- it cannot further reduce per-epoch time and yet the number of epochs grows significantly.

==> motivation.tex <==
\begin{table}[t]
    \setlength\arrayrulewidth{.5pt}
    \scriptsize\centering
   \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{c||c|c|c|c||c|c|c|c}
        \toprule
			& \multicolumn{4}{c||}{GNN Training with GPUs} & \multicolumn{4}{c}{GNN Training with CPUs}  \\ \cmidrule{2-5} \cmidrule{6-9}
        \textbf{$|E|$} & 
        \textbf{GPU} & \textbf{RAM(G)}   & \textbf{T(s)} & \textbf{C(\$)} &  \textbf{vCPU} & \textbf{RAM(G)}   & \textbf{T(s)} & \textbf{C(\$)}\\ \midrule
        0.5M           &    1$\times$1   & 3.2            &    \textbf{0.17}  & \textbf{0.0002}  &  1$\times$8     & 2        &    13.4  &  0.0006 \\ 
        1M             &    1$\times$1   & 4.3            &    \textbf{0.36}  & \textbf{0.0004}  &  1$\times$8     & 4        &    28.1  &  0.0013 \\ 
        2M             &    1$\times$4   & 23.9           &    \textbf{0.96}  & \textbf{0.001}   &  4$\times$8     & 32       &    61.0  &  0.0031 \\
        4M             &    4$\times$4   & $\thicksim$200$^\ast$ &  OOM      & $>$0.12$^\ast$ &  16$\times$8    & 209      &    \textbf{109.3} &  \textbf{0.04} \\\bottomrule    \end{tabular}
   \end{adjustbox}
    \vspace{-1.5em}
    \caption{Performance and costs of the modified DGL~\cite{dgl} when training graphs of varying sizes using GPUs and CPUs. Amazon EC2 g3.16xlarge instances (\$4.56/hr) are used as GPU servers while CPU servers are from c5.2xlarge (\$0.34/hr). Reported for each graph are the GPU/CPU resources used ($x\times y$ means $x$ nodes, each with $y$ GPUs/vCPUs), GPU/CPU memory needed (RAM), per-epoch time (T) and cost (C). Numbers annotated with $^\ast$ are estimated. \label{tab:cost-effiency}}
    \vspace{-2em}
\end{table}

\mysection{Extended Motivation \label{sec:motivation}}
We further motivate Lambda-based GNN training by comparing the time and costs of training with GPUs (g3.16xlarge) and CPUs (c5.2xlarge). For fair comparison, we ran DGL~\cite{dgl}, a popular GNN library (co-)developed by Amazon, over graphs of varying sizes generated from PaRMAT~\cite{parmat}, a parallel graph generator for graph mining~\cite{rmat-sdm04}. For training, we generated 25 labels and, for each vertex, a random feature vector with 100 features. Since the DGL does not perform distributed training, we partitioned the input graph using our partitioner (discussed later in \S\ref{sec:design}) and modified the DGL, turning it into a distributed system that trains over a graph partition on each node and synchronizes between nodes at each weight update. Updates from inter-partition edges are ignored in this version of the DGL to avoid a major re-design of the system (\ie, adding a \codeIn{Scatter} phase). Note that ignoring updates from these edges would not change the amount of tensor computation, which essentially always uses stale values from them. Also, using randomly generated features and labels is not an issue because the goal is to understand the performance and costs of computation, \emph{not} the accuracy.  

Table~\ref{tab:cost-effiency} reports comparison results. As shown, GPU-based training is two-orders-of-magnitude faster than CPU-based training when the number of edges is smaller than 4M.  Due to the huge performance gap, training with GPUs generates a lower cost even if the GPU instances have a much higher unit price.  However, when the 4M-edge graph is used, the amount of memory needed grows by almost 10$\times$ and even with 4 nodes each with 4 GPUs, the execution runs out of memory. This high memory requirement stems primarily from the quick growth of \emph{ghost vertices} (\ie, those whose incoming or outgoing edges are cut because of partitioning) on each node. All of these vertices need to be held in (GPU/CPU) memory for aggregation. As a result, we need $\thicksim$200GB memory ($\thicksim$30 GPUs) to train a GCN on this graph. 
In contrast, the CPU version completes the training on 16 nodes with a lower cost than the GPU version (if enough GPUs are given). 

The key takeaway here is although CPU-based training is scalable to large graphs, it is slow. By leveraging Lambdas for tensor-parallel computation, we aim to achieve a similar level of scalability and cost to that of CPU-based training while significantly boosting its performance. 


\iffalse
\mysection{Extended Motivation\label{sec:motivation}}
This section further motivates Lambda-based GNN training by comparing the time and costs of training with GPUs (g3.16xlarge) and CPUs (c5.2xlarge). To enable a fair comparison, we ran DGL~\cite{dgl}, a popular GNN library (co-)developed by Amazon, over graphs of varying sizes generated from PaRMAT~\cite{parmat}, a parallel graph generator for graph mining~\cite{rmat-sdm04}. For training, we generated 25 labels and, for each vertex, a random feature vector with 100 features. Since the DGL does not perform distributed training, we partitioned the input graph using our partitioner (discussed later in \S\ref{sec:design}) and modified the DGL, turning it into a distributed system that trains over a graph partition on each node and synchronizes between nodes at each weight update. Updates from inter-partition edges are ignored in this version of the DGL since supporting these edges would need a major re-design of the system (\ie, adding a \codeIn{Scatter} phase). Note that ignoring updates from these edges would not change the amount of tensor computation, which essentially always uses stale values from them. Using randomly generated features and labels is not an issue here because the goal is to understand the performance and costs of computation, \emph{not} the accuracy.  

Table~\ref{tab:cost-effiency} reports comparison results. As shown, GPU-based training is two-orders-of-magnitude more efficient than CPU-based training when the number of edges is smaller than 4M.  Due to the huge performance gap, training with GPUs generates a lower cost even if the GPU instances have a much higher unit price.  However, when the 4M-edge graph is used, the amount of memory needed grows by almost 10$\times$ and even with 4 nodes each with 4 GPUs, the GPU version still runs out of memory. This high memory requirement stems primarily from the quick growth of \emph{ghost vertices} (\ie, those whose incoming or outgoing edges are cut because of partitioning) on each node. All of these vertices need to be held in (GPU/CPU) memory for aggregation. As a result, we need $\thicksim$200GB memory ($\thicksim$30 GPUs) to train a GCN on this graph. 
In contrast, the CPU version completes the training on 16 nodes with a lower cost than the GPU version (if enough GPUs are given). 

The key takeaway here is although CPU-based training is scalable to large graphs, it is slow. By leveraging Lambdas for tensor-parallel computation, we aim to achieve a similar level of scalability and cost to that of CPU-based training while significantly boosting its performance. 
\fi


\begin{comment}
\MyPara{Problems with Adjacency Matrix.} GNN models are trained with deep learning frameworks such as TensorFlow or PyTorch and tested with relatively small graphs~\cite{kipf-iclr17, gan-iclr18, ggsnn-iclr16, graphsage-nips17}. The key technique in their implementations is to represent the graph as a sparse adjacency matrix, which, together with the dense feature matrix, is fed into a dataflow graph constructed in the framework. This approach works well on a single machine by piggybacking on the auto-gradient implementation as well as many optimizations in the framework. However, in a distributed setting, the matrix presentation of a graph can become a significant scalability-prohibiting obstacle for the following three reasons.  

\noindent \textit{Matrix partitioning.} To scale GNN training to large graphs, it is necessary to coordinate the partitioning of the graph's adjacency matrix $A$ and the vertex feature matrix $H$. Prior work \naively partitions the adjacency matrix into contiguous column chunks without considering the graph structure, causing the graph operations on partitions to involve unbalanced numbers of vertices. This also poses great challenges in the partitioning of the vertex feature matrix. As shown in Table~\ref{tab:naive-partition}, partitioning the Amazon graph into 8 contiguous chunks leads to an overall of \hx{X\%} duplicated vertex features and \hx{Y} GB extra memory consumption on each machine. To make matters worse, edge workloads are also imbalanced --- the chunk with fewest edges has only A edges while the chunk with most edges has B edges, leading to a \hx{C\%} workload difference.

\noindent\textit{Communication overhead.} Column (or rwo)-based partitioning of an adjacency matrix also leads to a large number of inter-partition dependencies, which incurrs large communication overhead during the \codeIn{Scatter} phase. Table~\ref{tab:naive-partition} shows that column-based partitioning of the Amazon graph across 8 machines leads to an average of inter-partition \hx{Z} edges; each \codeIn{Scatter} synchronizes \hx{X\%} vertices. 

\noindent \textit{Backward compatibility.}  During the backward phase, the adjacency matrix $A$ needs to be transposed. Backpropagation performs graph operations in a reverse direction, involving a very different set of vertices. This makes it harder to appropriately partition and manage the feature matrix. For example, partitioning needs to be re-done after the matrix transpose and re-distributed in a cluster setting. \hx{Can we add some data?}
\end{comment}




